Sanskrit Sandhi Splitting using seq2(seq)^2

In Sanskrit, small words (morphemes) are combined to form compound words through a process known as Sandhi. Sandhi splitting is the process of splitting a given compound word into its constituent morphemes. Although rules governing word splitting exists in the language, it is highly challenging to identify the location of the splits in a compound word. Though existing Sandhi splitting systems incorporate these pre-defined splitting rules, they have a low accuracy as the same compound word might be broken down in multiple ways to provide syntactically correct splits. In this research, we propose a novel deep learning architecture called Double Decoder RNN (DD-RNN), which (i) predicts the location of the split(s) with 95% accuracy, and (ii) predicts the constituent words (learning the Sandhi splitting rules) with 79.5% accuracy, outperforming the state-of-art by 20%. Additionally, we show the generalization capability of our deep learning model, by showing competitive results in the problem of Chinese word segmentation, as well.

==> 2_challenges.tex <==
\section{Challenges} \label{motiv}

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.35]{images/sandhiSplit.png}
	\caption{\label{exmotive}An example illustrating the different kinds of syntactical splits and the challenges for a sequence learning algorithm.}
	
\end{figure}
We summarize the major challenges in performing Sandhi splitting, as follows:

\begin{enumerate}
		\itemsep0em
	\item \textbf{Identifying multiple locations of split:} Identifying the location in a word where split has to be performed is the most challenging problem in performing splitting. As shown in Figure~\ref{exmotive}, transformation can happen in any location and in any form. Further, sandhi splitting involves identifying multiple potential locations, and validating them based on the previous locations. 
	\item \textbf{Cascading split effect:} There are some rules in which the effect of a split is not merely restricted to the immediate vicinity (neighboring characters). For example, in \textit{uttar\={a}ya\d{n}a} $\rightarrow$ \textit{uttara} + \textit{ayana}, the \textit{r} of \textit{uttara} changes the \textit{\d{n}} of \textit{ayana} to \textit{n}. 
	\item \textbf{Sam\={a}sa:} The process of \textit{Sam\={a}sa} is a process similar to Sandhi where words come together by discarding majority of their characters. A subset of the rules governing \textit{Sam\={a}sa} overlaps with Sandhi. Thus, Sandhi splitters need to maintain two rule sets to correctly identify the constituent words. Existing systems require the user to explicitly pass the intermediate results back to it to perform the splitting correctly. For example, existing systems correctly split the word with a \textit{Sam\={a}sa} \textit{lak\d{s}yasy\={a}rthatvavyavah\={a}r\={a}nurodhena} to form \textit{lak\d{s}yasya} + \textit{arthatvavyavah\={a}ra} + \textit{anurodhena}. However the second word, \textit{arthatvavyavah\={a}ra}, contains a Sandhi and must be sent back into the system to get its constituent words.
	\item \textbf{Incomplete rule set:} Though most of the splitting rules can easily be identified, there are many nuances which are often difficult to handle. There are also some rules which occur very rarely. For example, \textit{sa yog\={\i}} $\rightarrow$ \textit{sa\d{h}} + \textit{yog\={\i}}. Incomplete rule set during splitting will result in false negatives, such as, none of the existing splitters split (\textit{a} + \textit{chedya\d{h}} $\rightarrow$ \textit{acchedya\d{h}}), correctly as \textit{a} may not have the associated rule captured. Thus, heuristically defining all the splitting rules will be intractable, while learning them from examples is more generalizable.
\end{enumerate}

%%\subsection{Research Contributions}
%%In this research, we propose an approach for automated prediction of potential split locations in a compound word by using a deep attentional bidirectional character recurrent neural network (AB-RNN) with LSTM units. AB-RNN considers the compound word as a sequence of characters and provides a probability of split at each location of the sequence. The major research contributions are enumerated as follows:
%%\begin{enumerate}
%%	\item A novel sandhi split location prediction technique is proposed for compound words in Sanskrit using deep attentional bidirectional recurrent neural network (AB-RNN)~\cite{schuster1997bidirectional}~\cite{luong2015effective} with Long Short-Term Memory (LSTM) units~\cite{hochreiter1997long}. The proposed technique learns a character sequence embedding in a compound word and predicts the probability of a split occurring at a particular location given previous context (character sequence).
%%	
%%	\item To initiate and motivate reproducible research in this challenging problem, a large scale public benchmark dataset is created with a manually curated ground truth. Further, the source code of our approach is made public to enhance reproducibility.
%%	 
%%	\item Using the benchmark dataset, evaluate the performance of three publicly available tools on sandhi splitting: JNU sandhi splitter, UoH sandhi splitter, and Inria Sanskrit reader companion. Analysis of their results show the weakness of the existing tools and provides a direction of improvement. 
%%	
%%	\item Further, the proposed technique is compared against other standard deep learning approaches and the performances are benchmarked. The presence of attention mechanism improves the accuracy of split location prediction, as a larger context can be preserved and memorized.
%%
%%\end{enumerate}
%%
%%The rest of the paper is organized as follows: section 3 details the proposed benchmark dataset and the task of manual annotation while section 4 talks about existing sandhi splitting tools and similar works for Chinese. Section 5 explains the proposed deep learning based algorithm and section 6 discusses the experimental performance of the proposed approach. Finally, section 7 concludes the research and provides a direction for future work

















%\begin{table*}[t]
%	\begin{center}
%		\begin{tabular}{|p{1.2cm}|l|l|l|}
%			\hline 
%			\bf Criteria	& \bf Type	& \bf Explanation	& \bf Example \\
%			\hline
%			
%			\multirow{2}{*}{Position} & Internal &  Morphemes combine to form word &\textit{ bho} + \textit{anam}  $\rightarrow$ \textit{bhavanam } \\ \cline{2-4} 
%			
%			& External & Words combine to form compound words & \textit{tau} + \textit{ekad\={a}} $\rightarrow$ \textit{t\={a}vekad\={a}}  \\ \hline \hline
%			
%			\multirow{3}{*}{\parbox{1.2cm}{Type of character}} & Vowel &  Both joining letters are vowels  & \textit{ hima} + \textit{ \={a}laya\d{h}} $\rightarrow$ \textit{him\={a}laya\d{h}}  \\ \cline{2-4} 
%			
%			& Consonant &  One of the two letters is a consonant & \textit{v\d{r}k\d{s}a} + \textit{ch\={a}y\={a} } $\rightarrow$ \textit{v\d{r}k\d{s}acch\={a}y\={a}} 
%			\\ \cline{2-4}
%			
%			& Visarga &  Visarga with a vowel or a consonant &  \textit{ puna\d{h} } + \textit{janma } $\rightarrow$ \textit{punarjanma}    \\ \hline 
%			
%		\end{tabular}
%	\end{center}
%	\caption{\label{typestable} Different types of Sandhi classification}
%\end{table*}
%
%Based on the occurrence of Sandhi and the type of characters that happen during Sandhi merging and splitting, there are different classification of Sandhi as shown in Table~\ref{typestable}. Sandhi splitting involves an additional task of localizing the position at which the splits have to be made in a given word or compound word. Thus, designing a Sandhi splitter is considered more challenging than a Sandhi merger. Hence, most of the existing Sandhi splitters predict a ranked list of splits rather than a single split. A Sandhi splitter is typically evaluated in terms of accuracy when one of the members in the ranked list matches with the ground truth. However, the major challenged involved in evaluation is the lack of a golden dataset having manually annotated results of Sandhi splitting and Sandhi merging. The existing dataset, such as the University of Hyderabad (UoH) dataset\footnote{\url{http://sanskrit.uohyd.ac.in/Corpus/}}, has large scale but erroneous ground truth results making any evaluation performed in the dataset as not accurate. 
 

==> 3_existing.tex <==
\section{Existing Tools and Challenges} \label{relatmotiv}
In this section, we discuss the techniques used by the three most popular publicly available automated tools to perform Sandhi splitting. We also identify issues and challenges faced by these tools.

\subsection{JNU sandhi splitter}

This tool is specifically designed for a perticular class of Sandhi known as \textit{vowel based Sandhi}.~\cite{sachin2007sandhi}\footnote{Available at \url{http://sanskrit.jnu.ac.in/sandhi/viccheda.jsp}} Using a dictionary of possible morphemes, this tool, at every location recursively checks for binary splits. To be a valid split, both the left and right split segments must be available in the dictionary. If the second segment has more than one sound marked for Sandhi, then only the first segment is matched against the dictionary.

\subsection{UoH sandhi splitter}

\cite{kk} developed this tool at the Department of Sanskrit Studies, University of Hyderabad (UoH).\footnote{Available at \url{http://sanskrit.uohyd.ac.in/scl/}} This tool also recursively breaks a word at every possible position and applies appropriate Sandhi rules to generate possible morpheme candidates and passes them through a morphological analyzer. The split words are considered as valid only if all its constituents are recognized by the morphological analyzer. Weights are assigned to the accepted candidates and then ranked based on the descending order of weights.

\subsection{INRIA sanskrit reader companion}

\cite{huet2003}~\cite{goyal2013completeness} developed this tool at INRIA, France.\footnote{available at \url{http://sanskrit.inria.fr/DICO/reader.fr.html}} Initially, the word is analyzed to gather stems and their morphological parameters, such as permitted genders of nominal stems, allowed classes, and attested pre-verbs for roots. In the next stage, another round of stem generation is performed considering the various tenses, moods, absolutives, and participles in 10 varieties. Finally, inflexional morphology paradigms derive the inflected forms according to the morphological parameters, some of which are read from the word itself, while the others are defined in specific tables.

Comparison of these tools with our technique using the benchmark data set is provided in Section~\ref{eval}.

\iffalse
\subsection{Challenges} \label{motiv}

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.35]{images/sandhiSplit.png}
	\caption{\label{exmotive}An example illustrating the different kinds of syntactical splits and the challenges for a sequence learning algorithm.}
	
\end{figure}
We summarize the major challenges in performing Sandhi splitting, as follows:

\begin{enumerate}
		\itemsep0em
	\item \textbf{Identifying multiple locations of split:} Identifying the location in a word where split(s) must be performed is the most challenging problem in Sandhi splitting. As shown in Figure~\ref{fig:ex2}, transformation can happen in any location and in any form as shown in Figure~\ref{exmotive}. Further, sandhi splitting involves identifying multiple potential locations, and validating them based on the previous locations. 
	\item \textbf{Cascading split effect:} There are some rules in which the effect of a Sandhi is not merely restricted to the immediate vicinity (neighboring characters). For example, in \textit{uttar\={a}ya\d{n}a} $\rightarrow$ \textit{uttara} + \textit{ayana}, the \textit{r} of \textit{uttara} changes the \textit{\d{n}} of \textit{ayana} to \textit{n}. 
	\item \textbf{Sam\={a}sa:} The process of \textit{Sam\={a}sa} is a process similar to Sandhi where words come together by discarding majority of their characters. There is a significant overlapping in the way Sandhi  and \textit{Sam\={a}sa} rules are applied. Thus, Sandhi splitters need to maintain two rule sets to correctly identify the constituent words. Existing systems require the user to explicitly pass the intermediate results back to it to perform the splitting correctly. For example, the compound word  \textit{lak\d{s}yasy\={a}rthatvavyavah\={a}r\={a}nurodhena} with \textit{Sam\={a}sa}, can be split into \textit{lak\d{s}yasya} + \textit{arthatvavyavah\={a}ra} + \textit{anurodhena} using \textit{Sam\={a}sa} rules. After splitting the words, \textit{arthatvavyavah\={a}ra}, containing a Sandhi must be sent back into the system to get its constituent words.
	\item \textbf{Incomplete rule set:} Though most of the splitting rules can easily be identified, there are many nuances which are often difficult to handle. There are also some rules which occur very rarely. For example, \textit{sa yog\={\i}} $\rightarrow$ \textit{sa\d{h}} + \textit{yog\={\i}}. Incomplete rule set during splitting will result in false negatives, such as, none of the existing splitters split (\textit{a} + \textit{chedya\d{h}} $\rightarrow$ \textit{acchedya\d{h}}), correctly as \textit{a} may not have the associated rule captured. Thus, heuristically defining all the splitting rules will be intractable, while learning them from examples is more generalizable.
\end{enumerate}
\fi

==> 4_data.tex <==
\section{Data Curation} \label{datas}

Most automated algorithms in computational linguistics are data driven and require labelled data both for learning and evaluating models. Thus, the availability of a dataset is fundamental for research to be conducted in this domain. One of the contributions of this research is collating of a benchmark dataset from available repositories as listed below:
\begin{enumerate}
	\item \textbf{SandhiKosh} It is a  benchmark sandhi split corpus, developed by  \cite{sandhikosh}. This comprises of manually-annotated dataset as well as dataset from popular openware repositories such as UoH\footnote{Available at: \url{http://sanskrit.uohyd.ac.in/Corpus/}}. It consists of five different corpora which covers most of the sandhi rules specified in \Ast.
	
	\item \textbf{UoH subset} The corpus created by the University of Hyderabad\footnote{Available at: \url{http://sanskrit.uohyd.ac.in/Corpus/}} contains a total off $113,913$ words in the corpus with cases of typing errors, insufficient and incorrect splits. In SandhiKosh, there was stringent filtering of the split words applied, where as we considered flexible filtering.  We removed duplicate entries and restricted length of the compound word to an upper threshold of $31$ characters.  Finally, our filtered error free subset contains $67,183$ words and splits.
\end{enumerate}


 


For all our experiments, we converted the Sanskrit \textit{Devanagari} unicode script to \textit{Sanskrit Library Phonetic Basic encoding scheme (SLP1)}~\footnote{\url{https://en.wikipedia.org/w/index.php?title=SLP1}}. SLP1 maps each Sanskrit alphabet to a unique equivalent English character, ensuring that the transliteration between \textit{Devanagari} to \textit{SLP1} be unique.  We release\footnote{Link will be provided with the non-anonymized version of the paper} combined benchmark dataset of $71,747$ compound words along with their ground truth splits in SLP1 format. 


